ASASSN-15lh: A Superluminous Ultraviolet Rebrightening Observed by Swift and Hubble

We present and discuss ultraviolet and optical photometry from the Ultraviolet/Optical Telescope and X-ray limits from the X-Ray Telescope on Swift and imaging polarimetry and ultraviolet/optical spectroscopy with the Hubble Space Telescope of ASASSN-15lh. It has been classified as a hydrogen-poor superluminous supernova (SLSN I) more luminous than any other supernova observed. ASASSN-15lh is not detected in the X-rays in individual or coadded observations. From the polarimetry we determine that the explosion was only mildly asymmetric. We find the flux of ASASSN-15lh to increase strongly into the ultraviolet, with a ultraviolet luminosity a hundred times greater than the hydrogen-rich, ultraviolet-bright SLSN II SN 2008es. We find objects as bright as ASASSN-15lh are easily detectable beyond redshifts of ~4 with the single-visit depths planned for the Large Synoptic Survey Telescope. Deep near-infrared surveys could detect such objects past a redshift of ~20 enabling a probe of the earliest star formation. A late rebrightening -- most prominent at shorter wavelengths -- is seen about two months after the peak brightness, which is itself as bright as a superluminous supernova. The ultraviolet spectra during the rebrightening are dominated by the continuum without the broad absorption or emission lines seen in SLSNe or tidal disruption events and the early optical spectra of ASASSN-15lh. Our spectra show no strong hydrogen emission, showing only LyA absorption near the redshift previously found by optical absorption lines of the presumed host. The properties of ASASSN-15lh are extreme when compared to either SLSNe or tidal disruption events.

==> ASASSN-15lh_uvottable.tex <==
\begin{deluxetable*}{ccccccccc}
\tablecaption{Swift/UVOT Photometry of ASASSN-15lh\label{table_uvot}}
\tablehead{\colhead{Name} & \colhead{Filter} & \colhead{MJD} & \colhead{Mag} & \colhead{Mag Error} & \colhead{Upper Limit} & \colhead{Lower Limit} & \colhead{Rate} & \colhead{Rate Error}  \\ 
\colhead{} & \colhead{} & \colhead{(days)} & \colhead{} & \colhead{} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(counts s$^{-1}$)} & \colhead{(counts s$^{-1}$)} } 

%% All data must appear between the \startdata and \enddata commands
\startdata
ASASSN-15lh     & UVW2     & 57197.0974 &  15.555 &   0.066 &  20.993 &  11.085 &   5.371 &   0.327 \\
ASASSN-15lh     & UVW2     & 57199.7898 &  15.606 &   0.067 &  20.940 &  11.085 &   5.125 &   0.314 \\
ASASSN-15lh     & UVW2     & 57201.8196 &  15.764 &   0.067 &  20.844 &  11.085 &   4.430 &   0.274 \\
ASASSN-15lh     & UVW2     & 57205.6374 &  15.816 &   0.067 &  20.979 &  11.085 &   4.224 &   0.262 \\
ASASSN-15lh     & UVW2     & 57208.6638 &  16.006 &   0.068 &  20.945 &  11.085 &   3.544 &   0.223 \\
ASASSN-15lh     & UVW2     & 57211.6586 &  16.129 &   0.069 &  20.868 &  11.085 &   3.164 &   0.202 \\
ASASSN-15lh     & UVW2     & 57214.7125 &  16.345 &   0.087 &  19.985 &  11.085 &   2.593 &   0.207 \\
ASASSN-15lh     & UVW2     & 57216.5786 &  16.433 &   0.079 &  20.356 &  11.085 &   2.393 &   0.174 \\
ASASSN-15lh     & UVW2     & 57217.2487 &  16.442 &   0.066 &  21.648 &  11.085 &   2.372 &   0.144 \\
ASASSN-15lh     & UVW2     & 57217.6434 &  16.485 &   0.090 &  19.925 &  11.085 &   2.280 &   0.189 \\
ASASSN-15lh     & UVW2     & 57219.8033 &  16.653 &   0.096 &  19.846 &  11.085 &   1.954 &   0.173 \\
ASASSN-15lh     & UVW2     & 57220.5385 &  16.592 &   0.090 &  19.965 &  11.085 &   2.066 &   0.172 \\
ASASSN-15lh     & UVW2     & 57221.6849 &  16.615 &   0.079 &  20.523 &  11.085 &   2.022 &   0.148 \\
ASASSN-15lh     & UVW2     & 57223.5133 &  16.813 &   0.074 &  21.007 &  11.085 &   1.686 &   0.115 \\
ASASSN-15lh     & UVW2     & 57229.2672 &  17.157 &   0.078 &  20.971 &  11.085 &   1.228 &   0.088 \\
ASASSN-15lh     & UVW2     & 57232.8963 &  17.470 &   0.082 &  21.030 &  11.085 &   0.920 &   0.069 \\
ASASSN-15lh     & UVW2     & 57241.1244 &  17.745 &   0.078 &  21.391 &  11.085 &   0.714 &   0.051 \\
ASASSN-15lh     & UVW2     & 57244.8839 &  17.964 &   0.090 &  21.102 &  11.085 &   0.584 &   0.048 \\
ASASSN-15lh     & UVW2     & 57248.4721 &  18.098 &   0.083 &  21.438 &  11.085 &   0.516 &   0.039 \\
ASASSN-15lh     & UVW2     & 57250.7054 &  18.003 &   0.125 &  20.259 &  11.085 &   0.563 &   0.065 \\
ASASSN-15lh     & UVW2     & 57253.6979 &  18.141 &   0.140 &  20.157 &  11.085 &   0.496 &   0.064 \\
ASASSN-15lh     & UVW2     & 57255.6950 &  18.221 &   0.086 &  21.335 &  11.085 &   0.461 &   0.037 \\
ASASSN-15lh     & UVW2     & 57259.4036 &  18.412 &   0.115 &  20.792 &  11.085 &   0.387 &   0.041 \\
ASASSN-15lh     & UVW2     & 57262.7291 &  18.348 &   0.090 &  21.288 &  11.085 &   0.410 &   0.034 \\
ASASSN-15lh     & UVW2     & 57265.5618 &  18.505 &   0.215 &  19.607 &  11.085 &   0.355 &   0.070 \\
ASASSN-15lh     & UVW2     & 57268.7862 &  18.170 &   0.098 &  21.012 &  11.085 &   0.483 &   0.044 \\
ASASSN-15lh     & UVW2     & 57272.6061 &  18.205 &   0.090 &  21.242 &  11.085 &   0.468 &   0.039 \\
ASASSN-15lh     & UVW2     & 57272.8767 &  18.129 &   0.105 &  20.801 &  11.085 &   0.502 &   0.048 \\
ASASSN-15lh     & UVW2     & 57277.3583 &  17.825 &   0.076 &  21.537 &  11.085 &   0.664 &   0.047 \\
ASASSN-15lh     & UVW2     & 57282.8809 &  17.742 &   0.080 &  21.283 &  11.085 &   0.716 &   0.053 \\
ASASSN-15lh     & UVW2     & 57283.4095 &  17.787 &   0.081 &  21.222 &  11.085 &   0.687 &   0.051 \\
ASASSN-15lh     & UVW2     & 57284.3721 &  17.704 &   0.077 &  21.342 &  11.085 &   0.742 &   0.053 \\
ASASSN-15lh     & UVW2     & 57284.7725 &  17.712 &   0.079 &  21.263 &  11.085 &   0.737 &   0.054 \\
ASASSN-15lh     & UVW2     & 57290.8733 &  17.640 &   0.077 &  21.386 &  11.085 &   0.787 &   0.056 \\
ASASSN-15lh     & UVW2     & 57293.5673 &  17.496 &   0.077 &  21.234 &  11.085 &   0.899 &   0.064 \\
ASASSN-15lh     & UVW2     & 57296.6274 &  17.487 &   0.075 &  21.406 &  11.085 &   0.906 &   0.062 \\
ASASSN-15lh     & UVW2     & 57298.6449 &  17.469 &   0.074 &  21.429 &  11.085 &   0.921 &   0.063 \\
ASASSN-15lh     & UVW2     & 57299.5157 &  17.449 &   0.075 &  21.362 &  11.085 &   0.939 &   0.065 \\
ASASSN-15lh     & UVW2     & 57302.5733 &  17.488 &   0.075 &  21.316 &  11.085 &   0.905 &   0.063 \\
ASASSN-15lh     & UVW2     & 57305.4897 &  17.268 &   0.072 &  21.395 &  11.085 &   1.109 &   0.074 \\
ASASSN-15lh     & UVW2     & 57307.4522 &  17.223 &   0.077 &  21.066 &  11.085 &   1.155 &   0.082 \\
ASASSN-15lh     & UVW2     & 57309.6783 &  17.222 &   0.090 &  20.480 &  11.085 &   1.156 &   0.095 \\
ASASSN-15lh     & UVW2     & 57311.3086 &  17.134 &   0.080 &  20.810 &  11.085 &   1.254 &   0.092 \\
ASASSN-15lh     & UVW2     & 57313.2387 &  17.169 &   0.078 &  20.866 &  11.085 &   1.214 &   0.088 \\
ASASSN-15lh     & UVW2     & 57316.2410 &  17.192 &   0.076 &  21.078 &  11.085 &   1.189 &   0.083 \\
ASASSN-15lh     & UVW2     & 57317.7689 &  17.292 &   0.080 &  20.976 &  11.085 &   1.084 &   0.079 \\
ASASSN-15lh     & UVW2     & 57319.7639 &  17.364 &   0.079 &  21.063 &  11.085 &   1.015 &   0.074 \\
ASASSN-15lh     & UVW2     & 57325.3416 &  17.427 &   0.078 &  21.150 &  11.085 &   0.957 &   0.069 \\
ASASSN-15lh     & UVW2     & 57328.5299 &  17.198 &   0.074 &  21.150 &  11.085 &   1.182 &   0.081 \\
ASASSN-15lh     & UVW2     & 57330.1864 &  17.181 &   0.072 &  21.178 &  11.085 &   1.202 &   0.080 \\
ASASSN-15lh     & UVW2     & 57331.0591 &  17.135 &   0.076 &  20.939 &  11.085 &   1.254 &   0.088 \\
ASASSN-15lh     & UVW2     & 57334.5838 &  17.202 &   0.077 &  20.941 &  11.085 &   1.178 &   0.084 \\
ASASSN-15lh     & UVW2     & 57343.4378 &  17.278 &   0.078 &  21.034 &  11.085 &   1.099 &   0.079 \\
ASASSN-15lh     & UVW2     & 57346.1937 &  17.260 &   0.072 &  21.398 &  11.085 &   1.117 &   0.074 \\
ASASSN-15lh     & UVW2     & 57353.6315 &  17.167 &   0.119 &  19.632 &  11.085 &   1.216 &   0.134 \\
ASASSN-15lh     & UVW2     & 57356.2317 &  17.131 &   0.075 &  21.062 &  11.085 &   1.258 &   0.087 \\
ASASSN-15lh     & UVW2     & 57359.3198 &  17.194 &   0.077 &  20.928 &  11.085 &   1.187 &   0.084 \\
ASASSN-15lh     & UVW2     & 57362.8405 &  17.129 &   0.080 &  20.646 &  11.085 &   1.261 &   0.093 \\
ASASSN-15lh     & UVW2     & 57365.1007 &  17.219 &   0.082 &  20.664 &  11.085 &   1.160 &   0.088 \\
ASASSN-15lh     & UVW2     & 57366.3926 &  17.083 &   0.189 &  18.495 &  11.086 &   1.314 &   0.228 \\
ASASSN-15lh     & UVW2     & 57368.9556 &  17.261 &   0.078 &  20.836 &  11.085 &   1.116 &   0.080 \\
ASASSN-15lh     & UVW2     & 57371.4184 &  17.288 &   0.075 &  21.018 &  11.085 &   1.089 &   0.076 \\
ASASSN-15lh     & UVW2     & 57374.4071 &  17.424 &   0.080 &  20.853 &  11.085 &   0.960 &   0.071 \\
ASASSN-15lh     & UVW2     & 57377.1979 &  17.330 &   0.076 &  20.910 &  11.086 &   1.047 &   0.073 \\
ASASSN-15lh     & UVW2     & 57380.9236 &  17.423 &   0.080 &  20.754 &  11.086 &   0.962 &   0.071 \\
ASASSN-15lh     & UVW2     & 57383.2854 &  17.370 &   0.086 &  20.498 &  11.086 &   1.009 &   0.080 \\
ASASSN-15lh     & UVW2     & 57385.8720 &  17.348 &   0.132 &  19.428 &  11.086 &   1.030 &   0.126 \\
ASASSN-15lh     & UVW2     & 57393.6640 &  17.438 &   0.075 &  21.024 &  11.086 &   0.948 &   0.066 \\
ASASSN-15lh     & UVW2     & 57393.6640 &  17.438 &   0.075 &  21.024 &  11.086 &   0.948 &   0.066 \\
ASASSN-15lh     & UVW2     & 57396.7571 &  17.591 &   0.078 &  21.041 &  11.085 &   0.824 &   0.059 \\
ASASSN-15lh     & UVW2     & 57399.2511 &  17.506 &   0.077 &  20.951 &  11.086 &   0.891 &   0.063 \\
ASASSN-15lh     & UVW2     & 57427.7466 &  18.033 &   0.086 &  20.971 &  11.085 &   0.548 &   0.043 \\
ASASSN-15lh     & UVW2     & 57429.6501 &  18.183 &   0.105 &  20.562 &  11.086 &   0.477 &   0.046 \\
ASASSN-15lh     & UVW2     & 57433.5068 &  18.218 &   0.100 &  20.639 &  11.086 &   0.462 &   0.043 \\
ASASSN-15lh     & UVW2     & 57437.3219 &  18.203 &   0.095 &  20.733 &  11.086 &   0.469 &   0.041 \\
ASASSN-15lh     & UVW2     & 57447.4097 &  18.163 &   0.086 &  20.882 &  11.086 &   0.486 &   0.039 \\
ASASSN-15lh     & UVW2     & 57449.9336 &  18.152 &   0.105 &  20.499 &  11.086 &   0.491 &   0.048 \\
ASASSN-15lh     & UVW2     & 57450.1659 &  18.148 &   0.131 &  20.098 &  11.086 &   0.493 &   0.060 \\
ASASSN-15lh     & UVW2     & 57456.0811 &  18.110 &   0.086 &  21.053 &  11.085 &   0.510 &   0.040 \\
ASASSN-15lh     & UVW2     & 57457.6442 &  18.199 &   0.108 &  20.556 &  11.085 &   0.470 &   0.047 \\
ASASSN-15lh     & UVW2     & 57465.5588 &  18.254 &   0.085 &  21.135 &  11.086 &   0.447 &   0.035 \\
ASASSN-15lh     & UVW2     & 57470.3404 &  18.236 &   0.081 &  21.265 &  11.086 &   0.455 &   0.034 \\
ASASSN-15lh     & UVW2     & 57472.2258 &  18.270 &   0.149 &  20.029 &  11.085 &   0.441 &   0.061 \\
ASASSN-15lh     & UVW2     & 57475.6812 &  18.332 &   0.084 &  21.305 &  11.085 &   0.416 &   0.032 \\
ASASSN-15lh     & UVW2     & 57477.5496 &  18.308 &   0.109 &  20.648 &  11.085 &   0.425 &   0.043 \\
ASASSN-15lh     & UVW2     & 57480.3016 &  18.466 &   0.089 &  21.134 &  11.086 &   0.368 &   0.030 \\
ASASSN-15lh     & UVW2     & 57487.4805 &  18.590 &   0.142 &  20.297 &  11.086 &   0.328 &   0.043 \\
ASASSN-15lh     & UVW2     & 57489.0410 &  18.540 &   0.129 &  20.455 &  11.085 &   0.343 &   0.041 \\
ASASSN-15lh     & UVW2     & 57502.7087 &  18.444 &   0.103 &  20.803 &  11.086 &   0.375 &   0.036 \\
ASASSN-15lh     & UVW2     & 57505.3968 &  18.559 &   0.102 &  20.900 &  11.086 &   0.338 &   0.032 \\
ASASSN-15lh     & UVW2     & 57508.9296 &  18.537 &   0.127 &  20.451 &  11.086 &   0.345 &   0.040 \\
ASASSN-15lh     & UVW2     & 57511.8861 &  18.510 &   0.096 &  21.007 &  11.086 &   0.353 &   0.031 \\
ASASSN-15lh     & UVM2     & 57197.1005 &  15.240 &   0.062 &  20.358 &  10.555 &   4.405 &   0.252 \\
ASASSN-15lh     & UVM2     & 57199.7948 &  15.316 &   0.062 &  20.408 &  10.555 &   4.106 &   0.235 \\
ASASSN-15lh     & UVM2     & 57201.8228 &  15.464 &   0.063 &  20.349 &  10.555 &   3.584 &   0.210 \\
ASASSN-15lh     & UVM2     & 57205.6422 &  15.559 &   0.060 &  20.994 &  10.555 &   3.283 &   0.181 \\
ASASSN-15lh     & UVM2     & 57208.6673 &  15.736 &   0.061 &  20.984 &  10.555 &   2.791 &   0.156 \\
ASASSN-15lh     & UVM2     & 57211.6625 &  15.912 &   0.062 &  20.967 &  10.555 &   2.372 &   0.135 \\
ASASSN-15lh     & UVM2     & 57214.6771 &  15.978 &   0.070 &  20.265 &  10.555 &   2.232 &   0.144 \\
ASASSN-15lh     & UVM2     & 57214.7158 &  16.125 &   0.079 &  19.932 &  10.555 &   1.950 &   0.142 \\
ASASSN-15lh     & UVM2     & 57221.6920 &  16.498 &   0.070 &  20.682 &  10.554 &   1.383 &   0.090 \\
ASASSN-15lh     & UVM2     & 57223.5195 &  16.657 &   0.066 &  21.090 &  10.554 &   1.194 &   0.073 \\
ASASSN-15lh     & UVM2     & 57226.5226 &  16.907 &   0.069 &  21.064 &  10.554 &   0.949 &   0.060 \\
ASASSN-15lh     & UVM2     & 57229.2707 &  16.990 &   0.069 &  21.056 &  10.555 &   0.879 &   0.056 \\
ASASSN-15lh     & UVM2     & 57232.8995 &  17.250 &   0.073 &  21.100 &  10.554 &   0.692 &   0.047 \\
ASASSN-15lh     & UVM2     & 57241.1316 &  17.618 &   0.070 &  21.319 &  10.555 &   0.493 &   0.032 \\
ASASSN-15lh     & UVM2     & 57244.8908 &  17.700 &   0.079 &  21.020 &  10.555 &   0.457 &   0.033 \\
ASASSN-15lh     & UVM2     & 57248.4772 &  17.822 &   0.072 &  21.438 &  10.555 &   0.409 &   0.027 \\
ASASSN-15lh     & UVM2     & 57250.7105 &  17.891 &   0.113 &  20.297 &  10.555 &   0.383 &   0.040 \\
ASASSN-15lh     & UVM2     & 57253.6341 &  17.749 &   0.141 &  19.743 &  10.555 &   0.437 &   0.057 \\
ASASSN-15lh     & UVM2     & 57255.6647 &  18.015 &   0.106 &  20.554 &  10.555 &   0.342 &   0.033 \\
ASASSN-15lh     & UVM2     & 57259.4084 &  18.048 &   0.097 &  20.824 &  10.555 &   0.332 &   0.030 \\
ASASSN-15lh     & UVM2     & 57262.7322 &  18.124 &   0.079 &  21.352 &  10.555 &   0.309 &   0.023 \\
ASASSN-15lh     & UVM2     & 57268.7893 &  18.072 &   0.106 &  20.701 &  10.554 &   0.324 &   0.032 \\
ASASSN-15lh     & UVM2     & 57272.5701 &  17.807 &   0.112 &  20.288 &  10.555 &   0.414 &   0.043 \\
ASASSN-15lh     & UVM2     & 57272.8813 &  17.899 &   0.106 &  20.553 &  10.554 &   0.381 &   0.037 \\
ASASSN-15lh     & UVM2     & 57277.3295 &  17.591 &   0.084 &  20.892 &  10.554 &   0.505 &   0.039 \\
ASASSN-15lh     & UVM2     & 57282.8742 &  17.494 &   0.086 &  20.632 &  10.555 &   0.553 &   0.044 \\
ASASSN-15lh     & UVM2     & 57283.4050 &  17.340 &   0.082 &  20.632 &  10.555 &   0.637 &   0.048 \\
ASASSN-15lh     & UVM2     & 57284.3762 &  17.281 &   0.066 &  21.475 &  10.554 &   0.673 &   0.041 \\
ASASSN-15lh     & UVM2     & 57284.8418 &  17.326 &   0.086 &  20.603 &  10.554 &   0.645 &   0.051 \\
ASASSN-15lh     & UVM2     & 57290.8666 &  17.333 &   0.080 &  20.855 &  10.554 &   0.641 &   0.047 \\
ASASSN-15lh     & UVM2     & 57293.5577 &  17.018 &   0.076 &  20.798 &  10.554 &   0.857 &   0.060 \\
ASASSN-15lh     & UVM2     & 57296.6213 &  17.058 &   0.074 &  20.890 &  10.554 &   0.826 &   0.056 \\
ASASSN-15lh     & UVM2     & 57298.6517 &  17.096 &   0.065 &  21.467 &  10.555 &   0.797 &   0.048 \\
ASASSN-15lh     & UVM2     & 57299.5105 &  17.154 &   0.077 &  20.845 &  10.554 &   0.756 &   0.053 \\
ASASSN-15lh     & UVM2     & 57302.5696 &  17.051 &   0.073 &  20.824 &  10.555 &   0.831 &   0.056 \\
ASASSN-15lh     & UVM2     & 57305.4944 &  17.015 &   0.072 &  20.901 &  10.555 &   0.859 &   0.057 \\
ASASSN-15lh     & UVM2     & 57307.4586 &  16.961 &   0.069 &  21.064 &  10.555 &   0.903 &   0.057 \\
ASASSN-15lh     & UVM2     & 57309.6852 &  16.896 &   0.077 &  20.556 &  10.555 &   0.958 &   0.068 \\
ASASSN-15lh     & UVM2     & 57311.3134 &  16.775 &   0.069 &  20.827 &  10.555 &   1.072 &   0.068 \\
ASASSN-15lh     & UVM2     & 57313.2430 &  16.884 &   0.068 &  21.032 &  10.555 &   0.969 &   0.061 \\
ASASSN-15lh     & UVM2     & 57316.2334 &  16.933 &   0.080 &  20.388 &  10.555 &   0.927 &   0.068 \\
ASASSN-15lh     & UVM2     & 57317.7736 &  16.790 &   0.104 &  19.663 &  10.555 &   1.057 &   0.101 \\
ASASSN-15lh     & UVM2     & 57319.7568 &  17.068 &   0.083 &  20.480 &  10.555 &   0.818 &   0.062 \\
ASASSN-15lh     & UVM2     & 57322.7550 &  17.181 &   0.086 &  20.522 &  10.554 &   0.737 &   0.058 \\
ASASSN-15lh     & UVM2     & 57325.3339 &  17.174 &   0.083 &  20.421 &  10.555 &   0.742 &   0.057 \\
ASASSN-15lh     & UVM2     & 57328.5248 &  16.914 &   0.076 &  20.552 &  10.555 &   0.943 &   0.066 \\
ASASSN-15lh     & UVM2     & 57330.1905 &  16.901 &   0.070 &  20.877 &  10.555 &   0.954 &   0.061 \\
ASASSN-15lh     & UVM2     & 57331.0517 &  16.948 &   0.080 &  20.398 &  10.555 &   0.914 &   0.067 \\
ASASSN-15lh     & UVM2     & 57334.5768 &  17.002 &   0.082 &  20.318 &  10.555 &   0.869 &   0.066 \\
ASASSN-15lh     & UVM2     & 57343.4301 &  17.039 &   0.080 &  20.450 &  10.555 &   0.840 &   0.062 \\
ASASSN-15lh     & UVM2     & 57346.1984 &  16.945 &   0.080 &  20.479 &  10.555 &   0.916 &   0.067 \\
ASASSN-15lh     & UVM2     & 57349.2439 &  16.935 &   0.109 &  19.557 &  10.555 &   0.925 &   0.093 \\
ASASSN-15lh     & UVM2     & 57353.5619 &  16.917 &   0.089 &  20.071 &  10.555 &   0.940 &   0.077 \\
ASASSN-15lh     & UVM2     & 57356.2892 &  17.112 &   0.117 &  19.560 &  10.555 &   0.786 &   0.084 \\
ASASSN-15lh     & UVM2     & 57359.3127 &  17.048 &   0.082 &  20.352 &  10.555 &   0.833 &   0.063 \\
ASASSN-15lh     & UVM2     & 57362.8371 &  17.197 &   0.092 &  20.180 &  10.555 &   0.727 &   0.061 \\
ASASSN-15lh     & UVM2     & 57365.0929 &  17.160 &   0.084 &  20.378 &  10.555 &   0.752 &   0.058 \\
ASASSN-15lh     & UVM2     & 57368.9489 &  17.210 &   0.089 &  20.237 &  10.555 &   0.718 &   0.059 \\
ASASSN-15lh     & UVM2     & 57371.4246 &  17.206 &   0.083 &  20.528 &  10.555 &   0.720 &   0.055 \\
ASASSN-15lh     & UVM2     & 57374.3997 &  17.087 &   0.082 &  20.339 &  10.555 &   0.804 &   0.061 \\
ASASSN-15lh     & UVM2     & 57377.1896 &  17.195 &   0.083 &  20.322 &  10.555 &   0.728 &   0.056 \\
ASASSN-15lh     & UVM2     & 57380.9156 &  17.129 &   0.082 &  20.404 &  10.555 &   0.774 &   0.059 \\
ASASSN-15lh     & UVM2     & 57383.2888 &  17.461 &   0.118 &  19.846 &  10.555 &   0.570 &   0.062 \\
ASASSN-15lh     & UVM2     & 57385.8738 &  17.183 &   0.169 &  18.826 &  10.555 &   0.736 &   0.115 \\
ASASSN-15lh     & UVM2     & 57393.6663 &  17.284 &   0.083 &  20.518 &  10.555 &   0.670 &   0.051 \\
ASASSN-15lh     & UVM2     & 57396.7633 &  17.382 &   0.086 &  20.544 &  10.555 &   0.613 &   0.049 \\
ASASSN-15lh     & UVM2     & 57399.2553 &  17.358 &   0.084 &  20.582 &  10.555 &   0.626 &   0.048 \\
ASASSN-15lh     & UVM2     & 57427.7500 &  17.787 &   0.090 &  20.664 &  10.555 &   0.422 &   0.035 \\
ASASSN-15lh     & UVM2     & 57433.5093 &  17.813 &   0.102 &  20.412 &  10.555 &   0.412 &   0.039 \\
ASASSN-15lh     & UVM2     & 57437.3585 &  18.039 &   0.160 &  19.659 &  10.555 &   0.334 &   0.049 \\
ASASSN-15lh     & UVM2     & 57447.4127 &  17.922 &   0.088 &  20.798 &  10.555 &   0.373 &   0.030 \\
ASASSN-15lh     & UVM2     & 57449.9377 &  18.005 &   0.118 &  20.224 &  10.555 &   0.345 &   0.037 \\
ASASSN-15lh     & UVM2     & 57450.1701 &  18.138 &   0.164 &  19.727 &  10.555 &   0.305 &   0.046 \\
ASASSN-15lh     & UVM2     & 57454.2219 &  17.973 &   0.098 &  20.587 &  10.555 &   0.355 &   0.032 \\
ASASSN-15lh     & UVM2     & 57456.0858 &  18.023 &   0.103 &  20.560 &  10.555 &   0.340 &   0.032 \\
ASASSN-15lh     & UVM2     & 57465.5536 &  18.110 &   0.095 &  20.798 &  10.555 &   0.313 &   0.027 \\
ASASSN-15lh     & UVM2     & 57470.3330 &  17.994 &   0.086 &  20.904 &  10.555 &   0.349 &   0.028 \\
ASASSN-15lh     & UVM2     & 57472.2293 &  18.111 &   0.173 &  19.611 &  10.555 &   0.313 &   0.050 \\
ASASSN-15lh     & UVM2     & 57475.6723 &  18.016 &   0.089 &  20.936 &  10.555 &   0.342 &   0.028 \\
ASASSN-15lh     & UVM2     & 57477.5521 &  18.130 &   0.120 &  20.329 &  10.555 &   0.307 &   0.034 \\
ASASSN-15lh     & UVM2     & 57480.2968 &  18.294 &   0.099 &  20.869 &  10.555 &   0.265 &   0.024 \\
ASASSN-15lh     & UVM2     & 57487.4764 &  18.407 &   0.165 &  19.979 &  10.555 &   0.238 &   0.036 \\
ASASSN-15lh     & UVM2     & 57489.0314 &  18.274 &   0.144 &  20.171 &  10.555 &   0.269 &   0.036 \\
ASASSN-15lh     & UVM2     & 57499.7809 &  18.359 &   0.126 &  20.420 &  10.555 &   0.249 &   0.029 \\
ASASSN-15lh     & UVM2     & 57502.7010 &  18.374 &   0.127 &  20.420 &  10.555 &   0.246 &   0.029 \\
ASASSN-15lh     & UVM2     & 57505.3913 &  18.424 &   0.120 &  20.566 &  10.555 &   0.235 &   0.026 \\
ASASSN-15lh     & UVM2     & 57508.9488 &  18.350 &   0.108 &  20.761 &  10.555 &   0.251 &   0.025 \\
ASASSN-15lh     & UVM2     & 57511.8750 &  18.510 &   0.113 &  20.760 &  10.555 &   0.217 &   0.023 \\
ASASSN-15lh     & UVW1     & 57197.0939 &  15.265 &   0.060 &  20.519 &  11.145 &   7.410 &   0.408 \\
ASASSN-15lh     & UVW1     & 57199.7838 &  15.344 &   0.061 &  20.414 &  11.145 &   6.890 &   0.384 \\
ASASSN-15lh     & UVW1     & 57201.8162 &  15.403 &   0.061 &  20.367 &  11.146 &   6.529 &   0.367 \\
ASASSN-15lh     & UVW1     & 57205.6334 &  15.539 &   0.061 &  20.543 &  11.145 &   5.762 &   0.322 \\
ASASSN-15lh     & UVW1     & 57208.6610 &  15.724 &   0.062 &  20.487 &  11.146 &   4.858 &   0.276 \\
ASASSN-15lh     & UVW1     & 57211.6555 &  15.809 &   0.063 &  20.473 &  11.145 &   4.490 &   0.259 \\
ASASSN-15lh     & UVW1     & 57214.6686 &  15.924 &   0.066 &  20.283 &  11.145 &   4.038 &   0.246 \\
ASASSN-15lh     & UVW1     & 57214.7096 &  15.967 &   0.082 &  19.487 &  11.146 &   3.882 &   0.294 \\
ASASSN-15lh     & UVW1     & 57219.7891 &  16.238 &   0.071 &  20.168 &  11.146 &   3.025 &   0.197 \\
ASASSN-15lh     & UVW1     & 57221.6795 &  16.282 &   0.075 &  20.004 &  11.146 &   2.904 &   0.200 \\
ASASSN-15lh     & UVW1     & 57223.5083 &  16.411 &   0.067 &  20.493 &  11.146 &   2.580 &   0.160 \\
ASASSN-15lh     & UVW1     & 57226.5148 &  16.677 &   0.064 &  20.930 &  11.145 &   2.020 &   0.119 \\
ASASSN-15lh     & UVW1     & 57229.2644 &  16.741 &   0.072 &  20.492 &  11.145 &   1.903 &   0.126 \\
ASASSN-15lh     & UVW1     & 57232.8935 &  16.962 &   0.075 &  20.521 &  11.145 &   1.554 &   0.107 \\
ASASSN-15lh     & UVW1     & 57241.1186 &  17.226 &   0.070 &  20.948 &  11.145 &   1.217 &   0.079 \\
ASASSN-15lh     & UVW1     & 57244.8784 &  17.408 &   0.082 &  20.580 &  11.145 &   1.030 &   0.077 \\
ASASSN-15lh     & UVW1     & 57248.4679 &  17.428 &   0.073 &  20.912 &  11.145 &   1.011 &   0.068 \\
ASASSN-15lh     & UVW1     & 57250.7014 &  17.306 &   0.110 &  19.842 &  11.145 &   1.131 &   0.114 \\
ASASSN-15lh     & UVW1     & 57253.6677 &  17.478 &   0.098 &  20.176 &  11.146 &   0.965 &   0.087 \\
ASASSN-15lh     & UVW1     & 57255.6895 &  17.501 &   0.077 &  20.828 &  11.145 &   0.946 &   0.067 \\
ASASSN-15lh     & UVW1     & 57259.3996 &  17.594 &   0.097 &  20.350 &  11.145 &   0.868 &   0.078 \\
ASASSN-15lh     & UVW1     & 57262.7266 &  17.529 &   0.077 &  20.806 &  11.146 &   0.921 &   0.065 \\
ASASSN-15lh     & UVW1     & 57265.5583 &  17.492 &   0.083 &  20.610 &  11.145 &   0.953 &   0.073 \\
ASASSN-15lh     & UVW1     & 57268.7831 &  17.477 &   0.086 &  20.505 &  11.145 &   0.966 &   0.076 \\
ASASSN-15lh     & UVW1     & 57272.6007 &  17.376 &   0.076 &  20.739 &  11.146 &   1.060 &   0.074 \\
ASASSN-15lh     & UVW1     & 57272.8730 &  17.354 &   0.090 &  20.357 &  11.145 &   1.083 &   0.089 \\
ASASSN-15lh     & UVW1     & 57277.3518 &  17.159 &   0.070 &  20.716 &  11.146 &   1.295 &   0.083 \\
ASASSN-15lh     & UVW1     & 57282.8766 &  17.145 &   0.075 &  20.639 &  11.145 &   1.312 &   0.091 \\
ASASSN-15lh     & UVW1     & 57283.4068 &  17.111 &   0.074 &  20.616 &  11.146 &   1.354 &   0.093 \\
ASASSN-15lh     & UVW1     & 57284.3687 &  17.081 &   0.069 &  20.766 &  11.146 &   1.392 &   0.088 \\
ASASSN-15lh     & UVW1     & 57284.7694 &  17.119 &   0.074 &  20.605 &  11.146 &   1.344 &   0.091 \\
ASASSN-15lh     & UVW1     & 57290.8692 &  17.156 &   0.073 &  20.747 &  11.145 &   1.299 &   0.088 \\
ASASSN-15lh     & UVW1     & 57293.5617 &  16.996 &   0.072 &  20.714 &  11.145 &   1.505 &   0.100 \\
ASASSN-15lh     & UVW1     & 57296.6237 &  16.882 &   0.069 &  20.794 &  11.145 &   1.672 &   0.106 \\
ASASSN-15lh     & UVW1     & 57298.6395 &  17.015 &   0.068 &  20.923 &  11.145 &   1.479 &   0.092 \\
ASASSN-15lh     & UVW1     & 57299.5126 &  16.929 &   0.070 &  20.747 &  11.145 &   1.602 &   0.104 \\
ASASSN-15lh     & UVW1     & 57302.5710 &  16.971 &   0.069 &  20.757 &  11.146 &   1.540 &   0.098 \\
ASASSN-15lh     & UVW1     & 57305.4853 &  16.836 &   0.068 &  20.685 &  11.146 &   1.745 &   0.109 \\
ASASSN-15lh     & UVW1     & 57307.4468 &  16.886 &   0.072 &  20.516 &  11.146 &   1.665 &   0.111 \\
ASASSN-15lh     & UVW1     & 57311.3045 &  16.786 &   0.075 &  20.274 &  11.146 &   1.826 &   0.127 \\
ASASSN-15lh     & UVW1     & 57313.2353 &  16.767 &   0.073 &  20.329 &  11.146 &   1.859 &   0.125 \\
ASASSN-15lh     & UVW1     & 57316.2359 &  16.925 &   0.076 &  20.419 &  11.146 &   1.608 &   0.113 \\
ASASSN-15lh     & UVW1     & 57317.7273 &  17.000 &   0.076 &  20.471 &  11.146 &   1.499 &   0.104 \\
ASASSN-15lh     & UVW1     & 57319.7597 &  16.991 &   0.078 &  20.447 &  11.145 &   1.512 &   0.108 \\
ASASSN-15lh     & UVW1     & 57322.7247 &  16.744 &   0.134 &  18.939 &  11.145 &   1.898 &   0.234 \\
ASASSN-15lh     & UVW1     & 57325.3373 &  16.954 &   0.075 &  20.397 &  11.146 &   1.564 &   0.108 \\
ASASSN-15lh     & UVW1     & 57328.5266 &  16.726 &   0.070 &  20.225 &  11.147 &   1.930 &   0.125 \\
ASASSN-15lh     & UVW1     & 57330.1826 &  16.879 &   0.069 &  20.341 &  11.148 &   1.677 &   0.107 \\
ASASSN-15lh     & UVW1     & 57331.0545 &  16.805 &   0.075 &  20.060 &  11.148 &   1.795 &   0.124 \\
ASASSN-15lh     & UVW1     & 57334.5795 &  16.757 &   0.075 &  20.145 &  11.147 &   1.876 &   0.129 \\
ASASSN-15lh     & UVW1     & 57343.4334 &  16.917 &   0.074 &  20.491 &  11.146 &   1.619 &   0.110 \\
ASASSN-15lh     & UVW1     & 57346.1874 &  16.994 &   0.069 &  20.718 &  11.146 &   1.507 &   0.096 \\
ASASSN-15lh     & UVW1     & 57349.2151 &  16.858 &   0.076 &  20.325 &  11.146 &   1.709 &   0.120 \\
ASASSN-15lh     & UVW1     & 57353.5639 &  16.884 &   0.084 &  19.919 &  11.147 &   1.669 &   0.129 \\
ASASSN-15lh     & UVW1     & 57356.2272 &  16.948 &   0.076 &  20.348 &  11.146 &   1.574 &   0.110 \\
ASASSN-15lh     & UVW1     & 57359.3155 &  17.043 &   0.079 &  20.268 &  11.146 &   1.441 &   0.105 \\
ASASSN-15lh     & UVW1     & 57362.8383 &  16.921 &   0.081 &  20.075 &  11.146 &   1.613 &   0.121 \\
ASASSN-15lh     & UVW1     & 57365.0970 &  17.137 &   0.081 &  20.197 &  11.147 &   1.322 &   0.099 \\
ASASSN-15lh     & UVW1     & 57366.3914 &  17.069 &   0.080 &  20.086 &  11.147 &   1.407 &   0.104 \\
ASASSN-15lh     & UVW1     & 57368.9513 &  16.982 &   0.080 &  20.104 &  11.147 &   1.524 &   0.113 \\
ASASSN-15lh     & UVW1     & 57371.4114 &  17.110 &   0.077 &  20.138 &  11.148 &   1.355 &   0.096 \\
ASASSN-15lh     & UVW1     & 57374.4027 &  17.125 &   0.080 &  20.131 &  11.147 &   1.337 &   0.099 \\
ASASSN-15lh     & UVW1     & 57377.1930 &  17.240 &   0.084 &  19.780 &  11.152 &   1.203 &   0.093 \\
ASASSN-15lh     & UVW1     & 57380.9185 &  17.234 &   0.082 &  20.121 &  11.148 &   1.209 &   0.091 \\
ASASSN-15lh     & UVW1     & 57383.2812 &  17.263 &   0.095 &  19.761 &  11.148 &   1.178 &   0.103 \\
ASASSN-15lh     & UVW1     & 57385.8698 &  17.046 &   0.151 &  18.679 &  11.149 &   1.437 &   0.200 \\
ASASSN-15lh     & UVW1     & 57393.6610 &  17.260 &   0.077 &  20.242 &  11.148 &   1.181 &   0.083 \\
ASASSN-15lh     & UVW1     & 57396.7498 &  17.309 &   0.080 &  20.167 &  11.148 &   1.128 &   0.083 \\
ASASSN-15lh     & UVW1     & 57399.2468 &  17.379 &   0.081 &  20.164 &  11.148 &   1.058 &   0.079 \\
ASASSN-15lh     & UVW1     & 57427.7432 &  17.628 &   0.087 &  20.258 &  11.148 &   0.841 &   0.067 \\
ASASSN-15lh     & UVW1     & 57429.6464 &  17.853 &   0.115 &  19.859 &  11.148 &   0.683 &   0.072 \\
ASASSN-15lh     & UVW1     & 57433.5041 &  17.846 &   0.106 &  19.969 &  11.148 &   0.688 &   0.067 \\
ASASSN-15lh     & UVW1     & 57437.3176 &  17.819 &   0.098 &  20.150 &  11.148 &   0.705 &   0.063 \\
ASASSN-15lh     & UVW1     & 57447.4070 &  17.827 &   0.094 &  19.969 &  11.152 &   0.700 &   0.061 \\
ASASSN-15lh     & UVW1     & 57449.9293 &  17.995 &   0.150 &  19.253 &  11.159 &   0.600 &   0.083 \\
ASASSN-15lh     & UVW1     & 57450.1612 &  17.867 &   0.152 &  19.369 &  11.148 &   0.675 &   0.095 \\
ASASSN-15lh     & UVW1     & 57454.2142 &  17.915 &   0.099 &  20.137 &  11.148 &   0.645 &   0.059 \\
ASASSN-15lh     & UVW1     & 57456.0756 &  17.897 &   0.093 &  20.291 &  11.148 &   0.656 &   0.056 \\
ASASSN-15lh     & UVW1     & 57457.6397 &  17.974 &   0.122 &  19.916 &  11.147 &   0.611 &   0.068 \\
ASASSN-15lh     & UVW1     & 57465.5555 &  18.132 &   0.094 &  20.531 &  11.147 &   0.529 &   0.046 \\
ASASSN-15lh     & UVW1     & 57470.3361 &  17.947 &   0.083 &  20.673 &  11.147 &   0.627 &   0.048 \\
ASASSN-15lh     & UVW1     & 57472.2567 &  17.861 &   0.145 &  19.629 &  11.146 &   0.679 &   0.091 \\
ASASSN-15lh     & UVW1     & 57475.6755 &  17.950 &   0.084 &  20.771 &  11.146 &   0.625 &   0.048 \\
ASASSN-15lh     & UVW1     & 57477.5471 &  18.236 &   0.132 &  19.997 &  11.147 &   0.480 &   0.058 \\
ASASSN-15lh     & UVW1     & 57480.2987 &  18.175 &   0.094 &  20.576 &  11.147 &   0.508 &   0.044 \\
ASASSN-15lh     & UVW1     & 57487.4780 &  18.058 &   0.140 &  19.758 &  11.147 &   0.566 &   0.073 \\
ASASSN-15lh     & UVW1     & 57489.0351 &  18.329 &   0.142 &  20.087 &  11.146 &   0.441 &   0.058 \\
ASASSN-15lh     & UVW1     & 57499.7836 &  18.464 &   0.186 &  19.568 &  11.148 &   0.390 &   0.067 \\
ASASSN-15lh     & UVW1     & 57502.7037 &  18.288 &   0.124 &  20.103 &  11.147 &   0.458 &   0.052 \\
ASASSN-15lh     & UVW1     & 57505.3934 &  18.180 &   0.108 &  20.315 &  11.147 &   0.506 &   0.050 \\
ASASSN-15lh     & UVW1     & 57508.9529 &  18.160 &   0.098 &  20.518 &  11.146 &   0.515 &   0.047 \\
ASASSN-15lh     & UVW1     & 57511.8793 &  18.323 &   0.103 &  20.549 &  11.146 &   0.443 &   0.042 \\
ASASSN-15lh     & U        & 57197.0950 &  15.382 &   0.056 &  20.287 &  12.051 &  15.252 &   0.784 \\
ASASSN-15lh     & U        & 57199.7854 &  15.500 &   0.061 &  20.274 &  12.051 &  13.682 &   0.764 \\
ASASSN-15lh     & U        & 57201.8173 &  15.477 &   0.059 &  20.223 &  12.051 &  13.970 &   0.754 \\
ASASSN-15lh     & U        & 57205.6349 &  15.591 &   0.063 &  20.090 &  12.051 &  12.580 &   0.727 \\
ASASSN-15lh     & U        & 57208.6618 &  15.767 &   0.064 &  20.105 &  12.051 &  10.697 &   0.631 \\
ASASSN-15lh     & U        & 57211.6564 &  15.841 &   0.065 &  20.055 &  12.051 &   9.990 &   0.600 \\
ASASSN-15lh     & U        & 57214.6700 &  15.902 &   0.065 &  20.154 &  12.051 &   9.441 &   0.562 \\
ASASSN-15lh     & U        & 57214.7106 &  15.936 &   0.087 &  19.125 &  12.051 &   9.155 &   0.737 \\
ASASSN-15lh     & U        & 57216.3607 &  15.961 &   0.063 &  20.278 &  12.051 &   8.946 &   0.519 \\
ASASSN-15lh     & U        & 57216.4941 &  15.928 &   0.063 &  20.262 &  12.051 &   9.222 &   0.537 \\
ASASSN-15lh     & U        & 57216.7598 &  15.964 &   0.062 &  20.383 &  12.051 &   8.919 &   0.511 \\
ASASSN-15lh     & U        & 57220.5238 &  16.146 &   0.060 &  20.810 &  12.050 &   7.544 &   0.415 \\
ASASSN-15lh     & U        & 57221.6813 &  16.046 &   0.075 &  19.652 &  12.051 &   8.269 &   0.571 \\
ASASSN-15lh     & U        & 57223.5101 &  16.243 &   0.069 &  20.098 &  12.051 &   6.898 &   0.435 \\
ASASSN-15lh     & U        & 57226.5159 &  16.415 &   0.061 &  20.725 &  12.051 &   5.889 &   0.333 \\
ASASSN-15lh     & U        & 57229.2652 &  16.489 &   0.072 &  20.068 &  12.051 &   5.499 &   0.367 \\
ASASSN-15lh     & U        & 57232.8946 &  16.552 &   0.073 &  20.093 &  12.051 &   5.191 &   0.347 \\
ASASSN-15lh     & U        & 57241.1205 &  16.685 &   0.067 &  20.459 &  12.051 &   4.590 &   0.284 \\
ASASSN-15lh     & U        & 57244.8801 &  16.801 &   0.075 &  20.163 &  12.051 &   4.125 &   0.285 \\
ASASSN-15lh     & U        & 57248.4693 &  16.853 &   0.069 &  20.488 &  12.051 &   3.933 &   0.250 \\
ASASSN-15lh     & U        & 57250.7027 &  16.852 &   0.102 &  19.430 &  12.051 &   3.937 &   0.372 \\
ASASSN-15lh     & U        & 57253.6969 &  16.730 &   0.095 &  19.527 &  12.051 &   4.406 &   0.386 \\
ASASSN-15lh     & U        & 57255.6912 &  16.959 &   0.067 &  20.620 &  12.051 &   3.567 &   0.221 \\
ASASSN-15lh     & U        & 57259.4007 &  17.021 &   0.088 &  19.888 &  12.051 &   3.368 &   0.274 \\
ASASSN-15lh     & U        & 57262.7274 &  17.123 &   0.074 &  20.366 &  12.052 &   3.068 &   0.210 \\
ASASSN-15lh     & U        & 57265.5600 &  17.158 &   0.082 &  20.154 &  12.051 &   2.969 &   0.224 \\
ASASSN-15lh     & U        & 57268.7844 &  17.063 &   0.082 &  20.088 &  12.051 &   3.243 &   0.246 \\
ASASSN-15lh     & U        & 57272.6022 &  16.993 &   0.070 &  20.530 &  12.051 &   3.456 &   0.222 \\
ASASSN-15lh     & U        & 57272.8743 &  17.056 &   0.089 &  19.921 &  12.051 &   3.263 &   0.267 \\
ASASSN-15lh     & U        & 57277.3540 &  17.028 &   0.066 &  20.688 &  12.052 &   3.347 &   0.204 \\
ASASSN-15lh     & U        & 57282.8780 &  16.917 &   0.070 &  20.478 &  12.051 &   3.709 &   0.238 \\
ASASSN-15lh     & U        & 57283.4079 &  16.987 &   0.070 &  20.482 &  12.051 &   3.476 &   0.225 \\
ASASSN-15lh     & U        & 57284.3699 &  17.022 &   0.071 &  20.452 &  12.051 &   3.367 &   0.221 \\
ASASSN-15lh     & U        & 57284.7704 &  16.960 &   0.069 &  20.507 &  12.051 &   3.564 &   0.228 \\
ASASSN-15lh     & U        & 57290.8707 &  16.976 &   0.069 &  20.553 &  12.051 &   3.513 &   0.223 \\
ASASSN-15lh     & U        & 57293.5641 &  17.016 &   0.070 &  20.515 &  12.051 &   3.385 &   0.219 \\
ASASSN-15lh     & U        & 57296.6253 &  17.056 &   0.069 &  20.586 &  12.051 &   3.263 &   0.207 \\
ASASSN-15lh     & U        & 57298.6415 &  16.927 &   0.070 &  20.458 &  12.051 &   3.674 &   0.236 \\
ASASSN-15lh     & U        & 57299.5139 &  17.016 &   0.070 &  20.534 &  12.051 &   3.385 &   0.217 \\
ASASSN-15lh     & U        & 57302.5719 &  16.962 &   0.068 &  20.507 &  12.053 &   3.558 &   0.222 \\
ASASSN-15lh     & U        & 57305.4871 &  16.911 &   0.067 &  20.624 &  12.051 &   3.729 &   0.230 \\
ASASSN-15lh     & U        & 57307.4488 &  16.947 &   0.077 &  20.141 &  12.052 &   3.608 &   0.257 \\
ASASSN-15lh     & U        & 57309.6747 &  16.851 &   0.093 &  19.595 &  12.053 &   3.942 &   0.337 \\
ASASSN-15lh     & U        & 57311.3061 &  16.932 &   0.084 &  19.829 &  12.054 &   3.656 &   0.282 \\
ASASSN-15lh     & U        & 57313.2363 &  16.897 &   0.080 &  19.858 &  12.056 &   3.779 &   0.279 \\
ASASSN-15lh     & U        & 57316.2373 &  16.915 &   0.073 &  20.274 &  12.052 &   3.714 &   0.251 \\
ASASSN-15lh     & U        & 57317.7656 &  16.982 &   0.076 &  20.212 &  12.052 &   3.491 &   0.245 \\
ASASSN-15lh     & U        & 57319.7615 &  17.022 &   0.075 &  20.282 &  12.051 &   3.368 &   0.233 \\
ASASSN-15lh     & U        & 57325.3394 &  16.922 &   0.072 &  20.275 &  12.053 &   3.690 &   0.245 \\
ASASSN-15lh     & U        & 57328.5276 &  16.897 &   0.071 &  20.225 &  12.055 &   3.778 &   0.246 \\
ASASSN-15lh     & U        & 57330.1840 &  16.970 &   0.070 &  19.994 &  12.070 &   3.533 &   0.228 \\
ASASSN-15lh     & U        & 57331.0561 &  16.859 &   0.073 &  20.018 &  12.058 &   3.913 &   0.264 \\
ASASSN-15lh     & U        & 57334.5811 &  17.001 &   0.076 &  20.127 &  12.054 &   3.432 &   0.240 \\
ASASSN-15lh     & U        & 57343.4354 &  17.037 &   0.073 &  20.341 &  12.052 &   3.321 &   0.225 \\
ASASSN-15lh     & U        & 57346.1892 &  16.987 &   0.067 &  20.574 &  12.053 &   3.479 &   0.215 \\
ASASSN-15lh     & U        & 57349.2168 &  17.009 &   0.076 &  20.204 &  12.052 &   3.406 &   0.239 \\
ASASSN-15lh     & U        & 57353.5651 &  17.020 &   0.098 &  19.369 &  12.062 &   3.373 &   0.305 \\
ASASSN-15lh     & U        & 57356.2291 &  17.013 &   0.075 &  20.166 &  12.054 &   3.393 &   0.234 \\
ASASSN-15lh     & U        & 57359.3172 &  16.955 &   0.075 &  20.005 &  12.058 &   3.580 &   0.248 \\
ASASSN-15lh     & U        & 57362.8389 &  17.189 &   0.086 &  19.743 &  12.062 &   2.886 &   0.229 \\
ASASSN-15lh     & U        & 57365.0990 &  17.212 &   0.081 &  19.981 &  12.059 &   2.825 &   0.210 \\
ASASSN-15lh     & U        & 57366.4244 &  17.149 &   0.083 &  19.673 &  12.070 &   2.994 &   0.230 \\
ASASSN-15lh     & U        & 57368.9528 &  17.077 &   0.082 &  19.735 &  12.065 &   3.199 &   0.241 \\
ASASSN-15lh     & U        & 57371.4135 &  17.216 &   0.077 &  19.990 &  12.063 &   2.816 &   0.201 \\
ASASSN-15lh     & U        & 57374.4046 &  17.238 &   0.082 &  19.839 &  12.065 &   2.759 &   0.208 \\
ASASSN-15lh     & U        & 57377.1951 &  17.216 &   0.082 &  19.690 &  12.076 &   2.815 &   0.213 \\
ASASSN-15lh     & U        & 57380.9202 &  17.217 &   0.083 &  19.650 &  12.077 &   2.813 &   0.216 \\
ASASSN-15lh     & U        & 57383.2824 &  17.184 &   0.096 &  19.291 &  12.085 &   2.899 &   0.257 \\
ASASSN-15lh     & U        & 57385.8705 &  17.209 &   0.173 &  18.364 &  12.090 &   2.833 &   0.451 \\
ASASSN-15lh     & U        & 57393.6618 &  17.390 &   0.081 &  19.864 &  12.075 &   2.398 &   0.178 \\
ASASSN-15lh     & U        & 57396.7521 &  17.401 &   0.084 &  19.782 &  12.077 &   2.375 &   0.183 \\
ASASSN-15lh     & U        & 57399.2483 &  17.362 &   0.082 &  19.801 &  12.075 &   2.462 &   0.186 \\
ASASSN-15lh     & U        & 57427.7443 &  17.710 &   0.091 &  19.901 &  12.070 &   1.787 &   0.150 \\
ASASSN-15lh     & U        & 57429.6473 &  17.966 &   0.129 &  19.495 &  12.075 &   1.411 &   0.167 \\
ASASSN-15lh     & U        & 57433.5049 &  17.755 &   0.112 &  19.474 &  12.086 &   1.715 &   0.177 \\
ASASSN-15lh     & U        & 57437.3190 &  17.837 &   0.106 &  19.676 &  12.078 &   1.590 &   0.155 \\
ASASSN-15lh     & U        & 57447.4080 &  18.066 &   0.112 &  19.714 &  12.091 &   1.287 &   0.133 \\
ASASSN-15lh     & U        & 57449.9307 &  17.789 &   0.129 &  19.271 &  12.091 &   1.661 &   0.197 \\
ASASSN-15lh     & U        & 57450.1626 &  17.620 &   0.148 &  18.953 &  12.085 &   1.941 &   0.264 \\
ASASSN-15lh     & U        & 57454.2154 &  17.832 &   0.102 &  19.720 &  12.080 &   1.597 &   0.150 \\
ASASSN-15lh     & U        & 57456.0773 &  17.851 &   0.096 &  19.887 &  12.074 &   1.568 &   0.138 \\
ASASSN-15lh     & U        & 57457.6408 &  17.817 &   0.117 &  19.579 &  12.068 &   1.619 &   0.174 \\
ASASSN-15lh     & U        & 57465.5566 &  17.950 &   0.091 &  20.104 &  12.067 &   1.433 &   0.121 \\
ASASSN-15lh     & U        & 57470.3381 &  17.820 &   0.082 &  20.213 &  12.068 &   1.615 &   0.122 \\
ASASSN-15lh     & U        & 57472.2232 &  17.967 &   0.165 &  19.281 &  12.058 &   1.410 &   0.214 \\
ASASSN-15lh     & U        & 57475.6774 &  17.821 &   0.080 &  20.489 &  12.056 &   1.612 &   0.118 \\
ASASSN-15lh     & U        & 57477.5478 &  17.805 &   0.112 &  19.656 &  12.066 &   1.637 &   0.169 \\
ASASSN-15lh     & U        & 57480.2999 &  18.031 &   0.093 &  20.124 &  12.068 &   1.329 &   0.114 \\
ASASSN-15lh     & U        & 57487.4789 &  18.001 &   0.148 &  19.330 &  12.072 &   1.367 &   0.187 \\
ASASSN-15lh     & U        & 57489.0374 &  18.093 &   0.133 &  19.659 &  12.061 &   1.255 &   0.154 \\
ASASSN-15lh     & U        & 57502.7054 &  18.062 &   0.120 &  19.700 &  12.072 &   1.291 &   0.142 \\
ASASSN-15lh     & U        & 57505.3947 &  18.013 &   0.105 &  19.914 &  12.067 &   1.351 &   0.131 \\
ASASSN-15lh     & U        & 57508.9553 &  18.008 &   0.095 &  20.146 &  12.062 &   1.358 &   0.119 \\
ASASSN-15lh     & U        & 57511.8818 &  18.089 &   0.099 &  20.099 &  12.065 &   1.260 &   0.115 \\
ASASSN-15lh     & B        & 57197.0957 &  16.833 &   0.060 &  20.704 &  12.832 &   8.145 &   0.454 \\
ASASSN-15lh     & B        & 57199.7866 &  16.888 &   0.061 &  20.712 &  12.830 &   7.738 &   0.438 \\
ASASSN-15lh     & B        & 57201.8181 &  16.926 &   0.062 &  20.659 &  12.831 &   7.475 &   0.429 \\
ASASSN-15lh     & B        & 57205.6356 &  17.029 &   0.066 &  20.568 &  12.830 &   6.800 &   0.412 \\
ASASSN-15lh     & B        & 57208.6623 &  17.129 &   0.067 &  20.528 &  12.831 &   6.202 &   0.385 \\
ASASSN-15lh     & B        & 57211.6570 &  17.132 &   0.068 &  20.489 &  12.831 &   6.185 &   0.390 \\
ASASSN-15lh     & B        & 57214.6709 &  17.178 &   0.067 &  20.576 &  12.831 &   5.927 &   0.367 \\
ASASSN-15lh     & B        & 57214.7111 &  17.146 &   0.099 &  19.639 &  12.831 &   6.102 &   0.558 \\
ASASSN-15lh     & B        & 57221.6822 &  17.381 &   0.085 &  20.114 &  12.831 &   4.917 &   0.386 \\
ASASSN-15lh     & B        & 57223.5110 &  17.364 &   0.071 &  20.531 &  12.831 &   4.996 &   0.327 \\
ASASSN-15lh     & B        & 57226.5167 &  17.464 &   0.061 &  21.120 &  12.831 &   4.555 &   0.254 \\
ASASSN-15lh     & B        & 57229.2656 &  17.500 &   0.075 &  20.487 &  12.831 &   4.404 &   0.303 \\
ASASSN-15lh     & B        & 57232.8951 &  17.546 &   0.075 &  20.507 &  12.832 &   4.221 &   0.291 \\
ASASSN-15lh     & B        & 57241.1215 &  17.708 &   0.068 &  20.851 &  12.832 &   3.639 &   0.229 \\
ASASSN-15lh     & B        & 57244.8810 &  17.802 &   0.079 &  20.563 &  12.831 &   3.337 &   0.242 \\
ASASSN-15lh     & B        & 57248.4700 &  17.773 &   0.069 &  20.854 &  12.831 &   3.425 &   0.219 \\
ASASSN-15lh     & B        & 57250.7034 &  17.575 &   0.101 &  19.910 &  12.831 &   4.111 &   0.384 \\
ASASSN-15lh     & B        & 57253.6973 &  17.823 &   0.107 &  20.007 &  12.830 &   3.271 &   0.323 \\
ASASSN-15lh     & B        & 57255.6924 &  17.826 &   0.067 &  21.006 &  12.831 &   3.262 &   0.201 \\
ASASSN-15lh     & B        & 57259.4013 &  17.948 &   0.093 &  20.331 &  12.831 &   2.917 &   0.251 \\
ASASSN-15lh     & B        & 57262.7278 &  17.957 &   0.075 &  20.780 &  12.832 &   2.893 &   0.199 \\
ASASSN-15lh     & B        & 57265.5610 &  17.962 &   0.083 &  20.592 &  12.831 &   2.879 &   0.219 \\
ASASSN-15lh     & B        & 57268.7850 &  18.016 &   0.087 &  20.502 &  12.831 &   2.740 &   0.221 \\
ASASSN-15lh     & B        & 57272.6034 &  17.917 &   0.071 &  20.902 &  12.832 &   3.002 &   0.195 \\
ASASSN-15lh     & B        & 57272.8749 &  17.942 &   0.093 &  20.346 &  12.831 &   2.932 &   0.251 \\
ASASSN-15lh     & B        & 57277.3553 &  17.818 &   0.065 &  21.092 &  12.832 &   3.286 &   0.195 \\
ASASSN-15lh     & B        & 57284.3705 &  17.932 &   0.072 &  20.849 &  12.831 &   2.960 &   0.197 \\
ASASSN-15lh     & B        & 57284.7710 &  17.979 &   0.072 &  20.898 &  12.832 &   2.833 &   0.187 \\
ASASSN-15lh     & B        & 57298.6424 &  18.161 &   0.077 &  20.869 &  12.831 &   2.396 &   0.169 \\
ASASSN-15lh     & B        & 57305.4881 &  18.039 &   0.070 &  20.986 &  12.832 &   2.682 &   0.174 \\
ASASSN-15lh     & B        & 57307.4497 &  18.110 &   0.087 &  20.546 &  12.833 &   2.513 &   0.202 \\
ASASSN-15lh     & B        & 57309.6756 &  18.241 &   0.119 &  20.091 &  12.833 &   2.225 &   0.245 \\
ASASSN-15lh     & B        & 57311.3069 &  18.104 &   0.097 &  20.301 &  12.836 &   2.525 &   0.226 \\
ASASSN-15lh     & B        & 57313.2369 &  18.053 &   0.093 &  20.274 &  12.842 &   2.647 &   0.226 \\
ASASSN-15lh     & B        & 57317.7667 &  17.999 &   0.081 &  20.616 &  12.833 &   2.783 &   0.208 \\
ASASSN-15lh     & B        & 57330.1848 &  18.153 &   0.079 &  20.497 &  12.861 &   2.415 &   0.177 \\
ASASSN-15lh     & B        & 57346.1904 &  18.189 &   0.073 &  20.967 &  12.834 &   2.336 &   0.156 \\
ASASSN-15lh     & B        & 57366.4254 &  18.186 &   0.100 &  20.095 &  12.867 &   2.342 &   0.215 \\
ASASSN-15lh     & B        & 57371.4149 &  18.404 &   0.094 &  20.426 &  12.855 &   1.916 &   0.165 \\
ASASSN-15lh     & B        & 57383.2832 &  18.537 &   0.155 &  19.681 &  12.906 &   1.695 &   0.242 \\
ASASSN-15lh     & B        & 57385.8709 &  18.346 &   0.257 &  18.844 &  12.906 &   2.022 &   0.479 \\
ASASSN-15lh     & B        & 57393.6624 &  18.533 &   0.105 &  20.245 &  12.884 &   1.702 &   0.165 \\
ASASSN-15lh     & B        & 57396.7536 &  18.481 &   0.106 &  20.180 &  12.886 &   1.785 &   0.175 \\
ASASSN-15lh     & B        & 57399.2493 &  18.684 &   0.119 &  20.204 &  12.883 &   1.481 &   0.162 \\
ASASSN-15lh     & B        & 57427.7450 &  18.826 &   0.124 &  20.279 &  12.874 &   1.299 &   0.149 \\
ASASSN-15lh     & B        & 57429.6480 &  18.705 &   0.152 &  19.875 &  12.885 &   1.452 &   0.204 \\
ASASSN-15lh     & B        & 57433.5054 &  18.873 &   0.172 &  19.850 &  12.909 &   1.244 &   0.197 \\
ASASSN-15lh     & B        & 57437.3199 &  18.756 &   0.142 &  20.002 &  12.898 &   1.386 &   0.181 \\
ASASSN-15lh     & B        & 57447.4086 &  19.027 &   0.157 &  20.106 &  12.914 &   1.079 &   0.156 \\
ASASSN-15lh     & B        & 57449.9316 &  18.822 &   0.185 &  19.713 &  12.908 &   1.303 &   0.222 \\
ASASSN-15lh     & B        & 57450.1636 &  18.903 &   0.250 &  19.414 &  12.896 &   1.210 &   0.279 \\
ASASSN-15lh     & B        & 57454.2163 &  19.039 &   0.157 &  20.130 &  12.891 &   1.068 &   0.155 \\
ASASSN-15lh     & B        & 57456.0784 &  18.837 &   0.121 &  20.327 &  12.874 &   1.286 &   0.143 \\
ASASSN-15lh     & B        & 57457.6416 &  18.951 &   0.164 &  20.032 &  12.862 &   1.157 &   0.175 \\
ASASSN-15lh     & B        & 57472.2239 &  19.027 &   0.221 &  19.748 &  12.845 &   1.079 &   0.220 \\
ASASSN-15lh     & B        & 57477.5484 &  19.005 &   0.166 &  20.058 &  12.864 &   1.102 &   0.169 \\
ASASSN-15lh     & V        & 57197.0993 &  16.925 &   0.080 &  19.537 &  11.609 &   2.433 &   0.178 \\
ASASSN-15lh     & V        & 57199.7923 &  16.903 &   0.081 &  19.480 &  11.609 &   2.481 &   0.185 \\
ASASSN-15lh     & V        & 57201.8215 &  16.945 &   0.085 &  19.354 &  11.613 &   2.388 &   0.187 \\
ASASSN-15lh     & V        & 57205.6397 &  17.052 &   0.091 &  19.501 &  11.604 &   2.164 &   0.181 \\
ASASSN-15lh     & V        & 57208.6650 &  17.173 &   0.096 &  19.474 &  11.605 &   1.936 &   0.172 \\
ASASSN-15lh     & V        & 57211.6600 &  17.125 &   0.096 &  19.456 &  11.604 &   2.023 &   0.180 \\
ASASSN-15lh     & V        & 57214.6755 &  17.243 &   0.096 &  19.548 &  11.604 &   1.815 &   0.161 \\
ASASSN-15lh     & V        & 57214.7139 &  17.339 &   0.180 &  18.582 &  11.603 &   1.662 &   0.276 \\
ASASSN-15lh     & V        & 57221.6876 &  17.436 &   0.140 &  19.058 &  11.604 &   1.519 &   0.196 \\
ASASSN-15lh     & V        & 57223.5161 &  17.364 &   0.104 &  19.510 &  11.604 &   1.623 &   0.155 \\
ASASSN-15lh     & V        & 57226.5207 &  17.479 &   0.078 &  20.095 &  11.604 &   1.461 &   0.105 \\
ASASSN-15lh     & V        & 57229.2682 &  17.721 &   0.126 &  19.446 &  11.604 &   1.168 &   0.136 \\
ASASSN-15lh     & V        & 57232.8979 &  17.571 &   0.115 &  19.481 &  11.604 &   1.341 &   0.142 \\
ASASSN-15lh     & V        & 57241.1273 &  17.714 &   0.099 &  19.831 &  11.604 &   1.176 &   0.107 \\
ASASSN-15lh     & V        & 57244.8864 &  17.717 &   0.120 &  19.529 &  11.604 &   1.173 &   0.129 \\
ASASSN-15lh     & V        & 57248.4741 &  17.548 &   0.092 &  19.844 &  11.604 &   1.371 &   0.116 \\
ASASSN-15lh     & V        & 57250.7074 &  17.400 &   0.157 &  18.868 &  11.603 &   1.571 &   0.227 \\
ASASSN-15lh     & V        & 57253.6325 &  17.462 &   0.202 &  18.497 &  11.603 &   1.484 &   0.276 \\
ASASSN-15lh     & V        & 57255.6621 &  17.724 &   0.107 &  19.716 &  11.604 &   1.166 &   0.115 \\
ASASSN-15lh     & V        & 57259.4050 &  17.916 &   0.158 &  19.252 &  11.604 &   0.976 &   0.142 \\
ASASSN-15lh     & V        & 57262.7303 &  17.750 &   0.104 &  19.778 &  11.604 &   1.138 &   0.109 \\
ASASSN-15lh     & V        & 57268.7883 &  17.673 &   0.122 &  19.476 &  11.603 &   1.221 &   0.137 \\
ASASSN-15lh     & V        & 57272.5685 &  17.657 &   0.118 &  19.493 &  11.604 &   1.240 &   0.135 \\
ASASSN-15lh     & V        & 57272.8787 &  17.770 &   0.144 &  19.280 &  11.604 &   1.117 &   0.148 \\
ASASSN-15lh     & V        & 57277.3620 &  17.690 &   0.085 &  20.080 &  11.604 &   1.203 &   0.094 \\
ASASSN-15lh     & V        & 57284.3738 &  17.823 &   0.105 &  19.817 &  11.604 &   1.064 &   0.103 \\
ASASSN-15lh     & V        & 57284.7742 &  17.907 &   0.105 &  19.880 &  11.604 &   0.984 &   0.095 \\
ASASSN-15lh     & V        & 57298.6479 &  17.836 &   0.105 &  19.827 &  11.604 &   1.051 &   0.101 \\
ASASSN-15lh     & V        & 57305.4931 &  17.893 &   0.099 &  19.961 &  11.604 &   0.997 &   0.091 \\
ASASSN-15lh     & V        & 57307.4552 &  17.946 &   0.134 &  19.505 &  11.605 &   0.950 &   0.118 \\
ASASSN-15lh     & V        & 57309.6810 &  17.647 &   0.158 &  19.018 &  11.605 &   1.250 &   0.182 \\
ASASSN-15lh     & V        & 57311.3110 &  17.753 &   0.138 &  19.314 &  11.605 &   1.135 &   0.144 \\
ASASSN-15lh     & V        & 57313.2401 &  17.751 &   0.129 &  19.413 &  11.605 &   1.137 &   0.135 \\
ASASSN-15lh     & V        & 57317.7718 &  17.993 &   0.132 &  19.571 &  11.605 &   0.909 &   0.110 \\
ASASSN-15lh     & V        & 57330.1889 &  17.945 &   0.107 &  19.792 &  11.608 &   0.951 &   0.093 \\
ASASSN-15lh     & V        & 57346.1966 &  17.916 &   0.099 &  19.922 &  11.606 &   0.976 &   0.089 \\
ASASSN-15lh     & V        & 57371.4218 &  18.115 &   0.136 &  19.518 &  11.613 &   0.813 &   0.102 \\
ASASSN-15lh     & V        & 57383.2872 &  18.090 &   0.222 &  18.746 &  11.639 &   0.832 &   0.170 \\
ASASSN-15lh     & V        & 57385.8730 &    NULL &    NULL &  17.898 &  11.638 &   0.253 &   0.286 \\
ASASSN-15lh     & V        & 57393.6652 &  18.128 &   0.134 &  19.513 &  11.617 &   0.803 &   0.099 \\
ASASSN-15lh     & V        & 57396.7610 &  18.106 &   0.132 &  19.544 &  11.613 &   0.820 &   0.100 \\
ASASSN-15lh     & V        & 57399.2539 &  18.196 &   0.146 &  19.455 &  11.617 &   0.754 &   0.101 \\
ASASSN-15lh     & V        & 57427.7486 &  18.462 &   0.198 &  19.253 &  11.629 &   0.591 &   0.107 \\
ASASSN-15lh     & V        & 57429.6514 &  18.300 &   0.226 &  18.932 &  11.629 &   0.686 &   0.143 \\
ASASSN-15lh     & V        & 57433.5081 &  18.461 &   0.274 &  18.831 &  11.649 &   0.591 &   0.149 \\
ASASSN-15lh     & V        & 57437.3243 &  18.461 &   0.251 &  18.935 &  11.649 &   0.591 &   0.137 \\
ASASSN-15lh     & V        & 57447.4115 &  18.331 &   0.188 &  19.174 &  11.644 &   0.666 &   0.115 \\
ASASSN-15lh     & V        & 57449.9359 &  18.733 &   0.342 &  18.827 &  11.636 &   0.460 &   0.145 \\
ASASSN-15lh     & V        & 57450.1682 &    NULL &    NULL &  18.490 &  11.632 &   0.540 &   0.194 \\
ASASSN-15lh     & V        & 57454.2203 &  18.346 &   0.175 &  19.320 &  11.624 &   0.657 &   0.106 \\
ASASSN-15lh     & V        & 57456.0838 &  18.181 &   0.146 &  19.411 &  11.622 &   0.765 &   0.103 \\
ASASSN-15lh     & V        & 57457.8107 &    NULL &    NULL &  18.734 &  11.616 &   0.249 &   0.142 \\
ASASSN-15lh     & V        & 57472.2276 &  18.114 &   0.255 &  18.634 &  11.614 &   0.814 &   0.191 \\
ASASSN-15lh     & V        & 57477.5509 &  18.546 &   0.251 &  19.043 &  11.622 &   0.546 &   0.126 \\
\enddata

\tablecomments{Magnitudes are given in the UVOT/Vega system for easier comparison with other SNe published in that system (see \citealp{Brown_etal_2014_SOUSA} for a review).  The three $\sigma$ upper limits and lower (saturation) limits come from the exposure and background parameters.  Most of the photometry of ASASSN-15lh is not close to either of these limits, but they are given for completeness and easy comparison with other SN photometry tables from the Swift Optical/Ultraviolet Supernova Archive (SOUSA; \citealp{Brown_etal_2014_SOUSA}). 


\end{deluxetable*}



==> ASASSN-15lh_xrttable.tex <==

\begin{deluxetable}{cccc}

%% Keep a portrait orientation

%% Over-ride the default font size
%% Use Default (12pt)

%% Use \tablewidth{?pt} to over-ride the default table width.
%% If you are unhappy with the default look at the end of the
%% *.log file to see what the default was set at before adjusting
%% this value.

%% This is the title of the table.
\tablecaption{0.2 - 10 keV X-ray 3 Sigma Upper limits}


\tablehead{\colhead{MJD} & \colhead{Exposure} & \colhead{Flux Limit} & \colhead{Luminosity Limit} \\ 
\colhead{(days)} & \colhead{(s)} & \colhead{(ergs cm$^{-2}$ s$^{-1}$)} & \colhead{(ergs s$^{-1}$)} } 

%% All data must appear between the \startdata and \enddata commands
\startdata
57197.03 & 2484 & 1.024e-13 & 1.679e+43 \\


57197:57283 & 53548  & 1.006e-14 & 1.650e+42 \\
57283:57476 & 174086 & 6.257e-15 & 1.026e+42 \\
57197.03 & 2484 & 1.024e-13 & 1.679e+43 \\
57199.75 & 2354 & 1.432e-13 & 2.348e+43 \\
57201.75 & 2267 & 1.122e-13 & 1.840e+43 \\
57205.53 & 2874 & 1.171e-13 & 1.920e+43 \\
57208.60 & 2854 & 8.912e-14 & 1.461e+43 \\
57211.52 & 2667 & 9.538e-14 & 1.564e+43 \\
57214.64 & 1833 & 1.388e-13 & 2.276e+43 \\
57214.71 & 709 & 3.587e-13 & 5.882e+43 \\
57216.36 & 4052 & 8.047e-14 & 1.320e+43 \\
57216.49 & 172 & 1.476e-12 & 2.421e+44 \\
57216.76 & 219 & 1.158e-12 & 1.898e+44 \\
57217.11 & 2167 & 1.561e-13 & 2.560e+43 \\
57217.64 & 182 & 1.395e-12 & 2.288e+44 \\
57219.38 & 3536 & 7.194e-14 & 1.180e+43 \\
57219.68 & 277 & 9.177e-13 & 1.505e+44 \\
57220.49 & 2786 & 9.131e-14 & 1.497e+43 \\
57221.68 & 1505 & 1.689e-13 & 2.770e+43 \\
57223.47 & 2744 & 9.269e-14 & 1.520e+43 \\
57226.08 & 4627 & 5.497e-14 & 9.015e+42 \\
57229.13 & 2702 & 1.198e-13 & 1.965e+43 \\
57232.79 & 2749 & 9.252e-14 & 1.517e+43 \\
57241.05 & 4704 & 5.407e-14 & 8.866e+42 \\
57244.85 & 2951 & 8.618e-14 & 1.413e+43 \\
57248.36 & 4742 & 6.933e-14 & 1.137e+43 \\
57250.70 & 2237 & 1.514e-13 & 2.483e+43 \\
57253.57 & 941 & 3.607e-13 & 5.914e+43 \\
57255.62 & 3261 & 7.800e-14 & 1.279e+43 \\
57259.20 & 2457 & 1.035e-13 & 1.698e+43 \\
57262.59 & 4315 & 7.530e-14 & 1.235e+43 \\
57265.52 & 901 & 2.822e-13 & 4.627e+43 \\
57268.65 & 2212 & 1.150e-13 & 1.885e+43 \\
57272.43 & 2724 & 1.200e-13 & 1.967e+43 \\
57272.84 & 2322 & 1.095e-13 & 1.796e+43 \\
57277.28 & 4195 & 6.063e-14 & 9.943e+42 \\
57282.81 & 2549 & 9.977e-14 & 1.636e+43 \\
57283.07 & 2539 & 1.002e-13 & 1.643e+43 \\
57284.20 & 4719 & 5.390e-14 & 8.838e+42 \\
57284.60 & 3268 & 1.031e-13 & 1.690e+43 \\
57290.80 & 2831 & 1.192e-13 & 1.955e+43 \\
57293.52 & 2532 & 1.005e-13 & 1.647e+43 \\
57296.52 & 2971 & 8.560e-14 & 1.404e+43 \\
57298.57 & 4714 & 5.395e-14 & 8.848e+42 \\
57299.38 & 2809 & 9.055e-14 & 1.485e+43 \\
57302.43 & 3016 & 8.433e-14 & 1.383e+43 \\
57305.42 & 3708 & 1.293e-13 & 2.120e+43 \\
57307.34 & 2891 & 8.797e-14 & 1.443e+43 \\
57309.67 & 1478 & 2.289e-13 & 3.754e+43 \\
57311.27 & 2297 & 1.107e-13 & 1.816e+43 \\
57313.13 & 2672 & 9.520e-14 & 1.561e+43 \\
57316.21 & 1965 & 1.294e-13 & 2.123e+43 \\
57317.66 & 1885 & 1.797e-13 & 2.947e+43 \\
57319.72 & 1922 & 1.323e-13 & 2.169e+43 \\
57322.72 & 609 & 4.175e-13 & 6.846e+43 \\
57325.29 & 2130 & 1.869e-13 & 3.065e+43 \\
57328.28 & 2372 & 1.072e-13 & 1.758e+43 \\
57330.08 & 3848 & 6.610e-14 & 1.084e+43 \\
57331.02 & 1977 & 2.099e-13 & 3.442e+43 \\
57334.54 & 1855 & 1.371e-13 & 2.248e+43 \\
57343.40 & 2030 & 2.009e-13 & 3.294e+43 \\
57346.12 & 3546 & 7.174e-14 & 1.176e+43 \\
57349.18 & 1793 & 1.890e-13 & 3.098e+43 \\
57353.50 & 894 & 2.845e-13 & 4.666e+43 \\
57356.16 & 2025 & 1.256e-13 & 2.060e+43 \\
57359.28 & 1890 & 1.346e-13 & 2.207e+43 \\
57362.20 & 1488 & 1.709e-13 & 2.803e+43 \\
57365.06 & 1708 & 1.970e-13 & 3.230e+43 \\
57366.33 & 789 & 3.224e-13 & 5.286e+43 \\
57368.91 & 1763 & 1.443e-13 & 2.366e+43 \\
57371.38 & 2761 & 1.174e-13 & 1.925e+43 \\
57374.36 & 1947 & 1.306e-13 & 2.142e+43 \\
57377.16 & 2282 & 1.115e-13 & 1.828e+43 \\
57380.88 & 2032 & 1.251e-13 & 2.052e+43 \\
57383.15 & 1523 & 1.670e-13 & 2.738e+43 \\
57385.87 & 404 & 6.288e-13 & 1.031e+44 \\
57393.33 & 3268 & 7.782e-14 & 1.276e+43 \\
57396.71 & 2949 & 8.625e-14 & 1.414e+43 \\
57399.17 & 3056 & 8.322e-14 & 1.365e+43 \\
57427.68 & 3191 & 7.971e-14 & 1.307e+43 \\
57429.35 & 1955 & 1.301e-13 & 2.133e+43 \\
57433.07 & 2307 & 1.102e-13 & 1.808e+43 \\
57437.12 & 2242 & 1.134e-13 & 1.860e+43 \\
57447.24 & 3880 & 6.555e-14 & 1.075e+43 \\
57449.90 & 1780 & 1.429e-13 & 2.343e+43 \\
57450.16 & 951 & 2.674e-13 & 4.384e+43 \\
57453.95 & 3091 & 1.082e-13 & 1.775e+43 \\
57456.01 & 3223 & 1.272e-13 & 2.086e+43 \\
57457.48 & 1186 & 2.145e-13 & 3.517e+43 \\
57465.12 & 3391 & 9.888e-14 & 1.621e+43 \\
57470.23 & 4085 & 1.000e-13 & 1.640e+43 \\
57472.22 & 826 & 3.077e-13 & 5.047e+43 \\
57475.60 & 3743 & 6.796e-14 & 1.114e+43 \\
57477.21 & 1952 & 1.303e-13 & 2.136e+43 \\
57480.00 & 3356 & 7.579e-14 & 1.243e+43 \\
57487.11 & 1048 & 2.425e-13 & 3.977e+43 \\
\enddata

%% Include any \tablenotetext{key}{text}, \tablerefs{ref list},
%% or \tablecomments{text} between the \enddata and 
%% \end{deluxetable} commands

%% No \tablecomments indicated

%% No \tablerefs indicated

\end{deluxetable}


